Deep Generative Multimedia Children's Literature

Artistic work leveraging Machine Learning techniques is an increasingly popular endeavour for those with a creative lean. However, most work is done in a single domain: text, images, music, etc. In this work, I design a system for a machine learning created multimedia experience, specifically in the genre of children's literature. We detail the process for exclusively using publicly available pretrained deep neural network based models, I present multiple examples of the work my system creates, and I explore the problems associated in this area of creative work.

==> figs/diagram.tex <==

\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    % \begin{figure}
        \centering
        %\vspace{-5mm}
        \includegraphics[width=0.95\linewidth]{figures/diagram.png}
        \captionof{figure}{%\footnotesize{
        %Shared attributes across distinct and independently trained GANs. In (a), the top and bottom show aligned attribute of \texttt{hair-bangs} and \texttt{hair-color} respectively. In (b), the proposed method is able to find an unexpected \texttt{pencil-sketch} attribute direction in CelebA.}
         A diagram of my system architecture. An input prompt such as "A children's story about a boy and a horse." results in a video of a read story with music.} 
        %\vspace{2mm}
        \label{fig:diagram}
    % \end{figure}
\end{center}%
}]
